Learning Transformation Synchronization

Reconstructing the 3D model of a physical object typically requires us to align the depth scans obtained from different camera poses into the same coordinate system. Solutions to this global alignment problem usually proceed in two steps. The first step estimates relative transformations between pairs of scans using an off-the-shelf technique. Due to limited information presented between pairs of scans, the resulting relative transformations are generally noisy. The second step then jointly optimizes the relative transformations among all input depth scans. A natural constraint used in this step is the cycle-consistency constraint, which allows us to prune incorrect relative transformations by detecting inconsistent cycles. The performance of such approaches, however, heavily relies on the quality of the input relative transformations. Instead of merely using the relative transformations as the input to perform transformation synchronization, we propose to use a neural network to learn the weights associated with each relative transformation. Our approach alternates between transformation synchronization using weighted relative transformations and predicting new weights of the input relative transformations using a neural network. We demonstrate the usefulness of this approach across a wide range of datasets.

==> 04_algorithm_backup.tex <==
\section{Approach}
\label{Section:Overview}


The design of $\textup{Weight}_{\theta}$ combines three feed-forward sub-modules (See Figure~\ref{Figure:Network:Design}(a)). The first feed-forward sub-module
performs ICP alignment~\cite{Besl:1992:MRS} between $S_i$ and $S_j$ from the initial relative transformation described as $\overline{T}_{ij}^{(k)}:={T_j^{(k)}}\circ {T_i^{(k)}}^{-1}$:
\begin{equation}
(f_{ij}^{(k)}\in \{0,1\}, \hat{T}_{ij}^{(k)})\leftarrow \textup{ICP}(S_i, S_j, \overline{T}_{ij}^{(k)})
\label{Eq:ICP:Sub:Module}
\end{equation}
The output flag $f_{ij}^{(k)}$ indicates the success of ICP alignment, i.e., $f_{ij}^{(k)} = 0$ if ICP fails (e.g., non-overlap), and otherwise $f_{ij}^{(k)} = 1$. 

The second sub-module evaluates the quality of a rigid alignment $T_{ij}$ between $S_i$ and $S_j$:
\begin{equation}
o_{ij}\in \{0,1\} \leftarrow \textup{Score}_{\theta_s}(S_i, S_j, T_{ij}) 
\label{Eq:Scan:Score:Module}
\end{equation}
where the higher the $o_{ij}$, the better the pairwise match; $\theta_s$ denotes the trainable weights. As illustrated in Figure~\ref{Figure:Network:Design}(b), this sub-module first converts the rigid alignment into two heat maps $h(S_i,S_j,T_{ij})$ and $h(S_j,S_i,T_{ij}^{-1})$, where the value of each pixel of $h(S_i,S_j,T_{ij})$ equals the closest distance between the corresponding point in $S_i$ to points in $T_{ij}^{-1}(S_j)$. In other words, this distance is small for points in the overlapping region between $S_i$ and $S_j$. We then use a CNN with xxx layers and xxx fully connected layer to determine the output. Given $\textup{Score}$, we first apply it to the input relative transformation $T_{ij}^{\init}$, yielding $o_{ij}^{\init}$. Then if $f_{ij}^{(k)}=1$, we apply $\textup{Score}$ to $\hat{T}_{ij}^{(k)}$, yielding $o_{ij}^{(k)}$.

The third sub-module $\textup{Fuse}$ takes as input (1) the status vector $\bs{s}_{ij}^{(k)}$, (2) the ICP flag $f_{ij}^{(k)}$, and (3) the overlapping scores $o_{ij}^{(k)}$ and $o_{ij}^{\init}$, and computes the output of the pairwise matching module:
\small
\begin{equation}
(w_{ij}^{(k+1)},T_{ij}^{(k+1)}\in \{0,1\})  \leftarrow \textup{Fuse}_{\theta_f}(\bs{s}_{ij}^{(k)}, o_{ij}^{\init}, o_{ij}^{(k)}, f_{ij}^{(k)}) 
\label{Eq:Matching:Module}
\end{equation}
\normalsize
where $\theta_f$ denotes the trainable weights of $\textup{Fuse}$. 
As illustrated in Figure~\ref{Figure:Network:Design}(c), this sub-module consists xxx fully connected layers that output the weight $w_{ij}^{(k+1)}$ and an indicator $x_{ij}^{(k+1)}\in (0,1)$. The output relative transformation is then given by either the input relative transformation $\hat{T}_{ij}^{\init}$ or the ICP result $\hat{T}_{ij}^{(k)}$:
\begin{equation}
T_{ij}^{(k+1)} = x_{ij}^{(k+1)} \hat{T}_{ij}^{\init} + (1-x_{ij}^{(k+1)})\hat{T}_{ij}^{(k)}.
\end{equation}

With this setup, it remains to compute the derivatives of the status vectors $\bs{s}_{ij}^{(k)}$ and the spectral quantities (eigenvalues and eigenvectors) of $L^{(k)}$ with respect to variables of $L^{(k)}$, i.e., $w_{ij}^{(k)}, T_{ij}^{(k)}, (i,j)\in \set{E}$. For generality, we present the following propositions regarding a general Laplacian function $L(\bs{x})\in R^{N\times N}$

\begin{proposition} (\textbf{Eigenvalue derivative})
Let $\bs{u}_k$ be the k-th eigenvector of $L(\bs{0})$, then the derivative of the corresponding eigenvalue $\lambda_k(\bs{x})$ at $\bs{x} = \bs{0}$ is given by
\begin{equation}
\frac{\partial \lambda_k(\bs{x})}{\partial \bs{x}}|_{\bs{x} =\bs{0}} = \bs{u}_k^{T}\frac{\partial L(\bs{x})}{\partial \bs{x}}|_{\bs{x}=\bs{0}}\bs{u}_k.
\end{equation}
\end{proposition}

\begin{proposition}
(\textbf{Eigenvector derivative}) Let the eigen-decomposition of $L(\bs{x})$ as 
$$
L(\bs{x}) = U(\bs{x}) \Lambda(\bs{x}) U(\bs{x})^{T} + U_2(\bs{x}) \Lambda_2(\bs{x}) U_2(\bs{x})^{T},
$$
where $U(\bs{x})\in \R^{N\times K}$ and $U_2(\bs{x})\in \R^{N\times (N-K)}$, and 
$$
\Lambda(\bs{x}) =\textup{diag}(\lambda_1(\bs{x}),\cdots, \lambda_K(\bs{x})), \Lambda_2(\bs{x}) = \textup{diag}(\lambda_{K+1}(\bs{x}),\cdots, \lambda_{N}(\bs{x})).
$$

We assume there is a spectral gap, i.e., $\lambda_k < \lambda_{k+1}$.
Then the derivative of $U(\bs{x})$ with respect to each variable $x_i$ is given by
\footnotesize
$$
\frac{\partial U(\bs{x})}{\partial x_i}\bs{e}_k = (\lambda_i(\bs{0})-\Lambda_2(\bs{0}))^{-1}U_2(\bs{0})^{T}\frac{\partial L(\bs{x})}{\partial x_i}\bs{u}_k(\bs{0}),\ 1\leq k \leq K.
$$
\normalsize
\end{proposition}
Note that we have omitted a term $UX$ in the gradient term, where $X$ is a skew-symmetric matrix. However, this term does not contribute to the gradient of resulting gradient of the absolute poses. 

\begin{proposition}
(\textbf{Psuedo-Inverse derivative}) The derivative of the pseudo-inverse of $L(\bs{x})$ is given by? Let us just try derivative of a positive definite matrix first:
$$
\frac{\partial L^{-1}(\bs{x})}{\partial x_i}|_{\bs{x} = \bs{0}} = L(\bs{0})^{-1}\frac{\partial L(\bs{x})}{\partial x_i}|_{\bs{x} =\bs{0}}L(\bs{0})^{-1}.
$$
\end{proposition}

The derivative of SVD can also be computed. Consider
$$
A = U\Sigma V^T.
$$
Let us parameterize $\frac{\partial U}{\partial \theta}$ and $\frac{\partial V}{\partial \theta}$ as follows
$$
\frac{\partial U}{\partial \theta} = U\cdot X, \quad \frac{\partial V}{\partial \theta} = V\cdot Y,
$$
where both $X$ and $Y$ are skew-asymmetric matrices. 
It follows that 
$$
\frac{\partial (UV^T)}{\partial \theta} = U(X-Y)V^{T}.
$$

On the other hand, we can solve $X$ and $Y$ from
$$
U^{T}\frac{\partial A}{\partial \theta}V = X\Sigma - \Sigma Y + \frac{\partial \Sigma}{\partial \theta}.
$$
In fact $\forall i < j$,
$$
x_{ij} - y_{ij} = \frac{\bs{u}_i^{T}\frac{\partial A}{\partial \theta}\bs{v}_j -\bs{u}_j^{T}\frac{\partial A}{\partial \theta}\bs{v}_i}{\sigma_i + \sigma_j}
$$

In this section, we formally state the transformation synchronization problem studied in this paper and present the technical details of our approach. We begin with the problem statement and approach overview in Section~\ref{Section:Problem:Statement}. We then discuss the two major modules of our approach, namely the optimization module and the weighting module in Section~\ref{Section:Optimization:Module} and Section~\ref{Section:Weighting:Module}, respectively.

\subsection{Problem Statement and Approach Overview}
\label{Section:Problem:Statement}

Consider $n$ input scans $\set{S} = \{S_i, 1\leq i \leq n\}$ capturing the same underlying object from different camera poses. Let $\Sigma_i$ denote the local coordinate system associated with $S_i$. The input to transformation synchronization is given by model graph $\set{G} = (\set{S}, \set{E})$. Each edge $(i,j)\in \set{E}$ of the model graph is associated with a relative transformations $T_{ij}^{\init}\in SE(3)$ pre-computed using an off-the-shelf algorithm. It is expected that a significant portion of these relative transformations are corrupted. The goal of transformation synchronization is to estimate the pose $T_i\in SE(3)$ of these scans in a world coordinate system $\Sigma$. Without losing generality, we assume the world coordinate system is given by $\Sigma:=\Sigma_1$. 


Our approach combines two key ideas for transformation synchronization. The first idea is to introduce a weight $w_{ij}$ associated with edge $(i,j)\in \set{E}$. 

Specifically, our approach maintains for each scan $S_i$ a candidate transformation set $\set{T}_i = \{T_{i,1},\cdots, T_{i,K}\}$. The size $K$ of set is pre-defined. We initialize each $\set{T}_i$ using the leading $4K$ singular values/vectors of the data matrix that stores $T_{ij}^{\init}$ in blocks. Our approach also maintains a weight $w_{ij}$ for edge. These edge weights are updated using a neural network. 

Our approach alternates between an optimization phase and and a weighting phase. In the optimization phase, the edge weights $w_{ij}$ are fixed and we optimize the candidate pose sets $\set{T}_{i}$. In the weighting phase, we fix the candidate pose sets $\set{T}_i$ and use a neural network to update the edge weights. This process is iterated. We also implement the entire pipeline as an end-to-end network and train it on labeled data. 


\subsection{Optimization Module}
\label{Section:Optimization:Module}

In the optimization module, we optimize the candidate pose set by following continuous optimization problem:
\begin{align}
\underset{\set{T}_i, y_{ijk}}{\textup{minimize}} &\quad  \sum\limits_{(i,j)\in \set{E}} \sum\limits_{k=1}^{K} y_{ijk}\|T_{ij} - T_{j,k} \cdot T_{i,k}^{-1}\|_{\set{F}}^2 \nonumber \\
\textup{subject to} & \quad \sum\limits_{k=1}^{K} y_{ijk} = 1,\quad (i,j)\in \set{E} \nonumber \\
& \quad y_{ijk}\geq 0,\ (i,j)\in \set{E}, \ 1\leq k \leq K.
\end{align}

For optimization, we alternate between optimizing $y_{ijk}$ and fixing $y_{ijk}$ to optimize the latent variables $\set{T}_i$. Both steps admit closed-form solutions. 

\subsection{Weighting Module}
\label{Section:Weighting:Module}

In the weighting module, we train a neural network that takes as input a pair of scans $S_i$ and $S_j$, the candidate pose sets $\set{T}_i$ and $\set{T}_j$, and the input relative pose $T_{ij}^{\init}$, and outputs a score $w_{ij}$:
$$
w_{ij}\leftarrow w(S_i,S_j,T_{ij}^{\init}, \set{T}_i, \set{T}_j).
$$

\subsection{A Simplified Model}

We should start from the case $K=1$, and this is the baseline to compare. Let $\bs{w}$ collect the edge weights. Denote the weighted data matrix $X(\bs{w})$ whose blocks are
\begin{align}
X_{ij}(\bs{w}) = \left\{
\begin{array}{cc}
w_{ij}T_{ij} & (i,j)\in \set{E} \\
0 & \textup{otherwise}
\end{array}
\right.\
\end{align}

Let $X(\bs{w}) = U\Lambda V^{T}$ be the singular value decomposition of the weighted data matrix, where $U,V\in \R^{4n\times 4}$ and $\Lambda \in \R^{4\times 4}$. Consider $T_i = (\bs{e}_i\otimes I_4)^T\Lambda V^{T}(\bs{e}_1\otimes I_4)$. We round $T_i$ into $SE(3)$ by first performing SVD on $T_i(1:3,1:3)$. We scale this so that the singular values of the scaled block is close to $1$. 

The neural network determines the network weight via
$$
w_{ij}\leftarrow w(S_i,S_j,T_{ij}^{\init}, T_j^{(k)}{T_i^{(k)}}^{-1}).
$$
Essentially, $w_{ij}$ is set to zero if there is a nice match close to $T_j^{(k)}{T_i^{(k)}}^{-1}$ and $T_j^{(k)}{T_i^{(k)}}^{-1}$ is far from $T_{ij}^{\init}$.

This learning approach is expected to be better than non-deep learning based approaches. 

Increasing $K$ shall give us better intermediate solutions $\set{T}_i$, and more chances to kill bad matches. There are $K^2$ candidate relative poses per pair. 


\subsection{Spectral Transformation Synchronization}


Consider an observation graph $\set{G} = (\set{V},\set{E})$, where $\set{V}$ and $\set{E}$ denote the vertex and edge sets, respectively. Let $R_{ij}^{\init}$ and $\bs{t}_{ij}^{\init}$ be the rotation and translation associated with each edge $(i,j)\in \set{E}$. Consider a weight $w_{ij}\in (0,1)$ associated with each edge as well. Our approach for transformation synchronization considers two sequential steps, where the first step estimates the rotation component per object, and where the second step estimates the translation component. Specifically, we the first component considers a data matrix $R \in \R^{3n \times 3n}$, where
$$
R_{ij} = \left\{
\begin{array}{cc}
\frac{w_{ij}}{\sqrt{d_i(\bs{w}) d_j(\bs{w})}}R_{ij}^{\init} & (i,j)\in \set{E} \\
0 & \textup{otherwise}
\end{array}
\right.\
$$
where
$$
d_i(\bs{w}) = \sum\limits_{j\in \set{N}(i)} w_{ij}.
$$

Let $U = (U_1^{T},\cdots, U_n^{T})^{T}\in \R^{3n\times 3}$ be the leading eigenvectors of $R$. We compute the rotation synchronization result as 
$$
R_i^{\star} = V_i W_i^{T},\quad U_i U_1^{T} = V_i \Sigma_i W_i^{T}, \quad 1\leq i \leq n.
$$
After predicting the rotations, we solve the following least square problem to estimate the translations:

\begin{align}
\underset{\bs{t}_i, 1\leq i \leq n}{\textup{minimize}} & \quad \sum\limits_{(i,j)\in \set{E}} \ w_{ij}\|R_{ij}^{\init}\bs{t}_i+\bs{t}_{ij}^{\init}-\bs{t}_j\|^2 \nonumber \\
\textup{subject to} &\quad \sum\limits_{i=1}^{n} \bs{t}_i = 0
\end{align}

Given the optimal solutions $(R_i^{\star}, \bs{t}_i^{\star}), 1\leq i \leq n$, we determine the weight at the next iteration as
\begin{equation}
w_{ij}:= \left\{
\begin{array}{cc}
1 & \|R_{ij}^{\init}R_i^{\star} -R_j^{\star}\|_{\set{F}}^2 + \mu \|\|^2 \leq c \delta ^k \\
0 & \textup{otherwise}
\end{array}
\right.\
\end{equation}
where $\delta < 1$. 



==> 07_analysis.tex <==
\section{Analysis}
\label{Section:Analysis}
Section \ref{Section:Noise:Model} introduce the noise model, section \ref{Section:Exact:Recovery} establish the results under noise free setting, then section \ref{Section:Main:Result} considers the noisy setting.

\subsection{Noise Model} \label{Section:Noise:Model}
Assume the ground truth rotation being $R_1^{\star}, R_2^{\star}, \ldots, R_n^{\star}$, we consider the following non-uniform noise on the measured correspondence
\begin{equation}
    R_{ij} = (R_j^{\star})^T (I + N_{ij}) R_i^{\star}, \quad \|N_{ij}\| \leq \begin{cases}
        \sigma & \textup{ w.p. } p \\
        C & \textup{ w.p. } 1-p \\
    \end{cases}
\label{eq:Noise}
\end{equation}
where $C \gg \sigma$.

\subsection{Exact Recovery}\label{Section:Exact:Recovery}
In this subsection, we show that algorithm \ref{Alg:truncated:laplacianRS} indeed recovers the perfect rotation in the noise free setting.
\begin{proposition}
    If $N_{ij} = 0$ in \eqref{eq:Noise}, i.e. $R_{ij} = (R_j^{\star})^T R_i^{\star}$, then algorithm \ref{Alg:truncated:laplacianRS} outputs $R_i = Q^T R_i^{\star}$, where $Q$ is another rotation matrix.
\end{proposition}
\begin{proof}
    See Appendix \ref{Appendix:A}.
\end{proof}

\subsection{Main Result}\label{Section:Main:Result}

==> 08_plan.tex <==
\section{Plan}
\label{Section:Plan}

\begin{itemize}

\item \yao{-Page 2, 109: RGBD seems not definite earlier}

\item \yao{-There is a bit gap: from before “in this paper, we introduce“ to after. Earlier we talked about “heavily depends on the noise pattern”, then it becomes “formulate the transformation synchronization as an end-to-end neural networks”. It is not clear to me why this formulation can address this problem.}

\item \yao{-A message from these exact recovery conditions is that
existing methods only work if the fraction of noise in the
input  relative  transformations  is  below  a  threshold}

\item \yao{-Do you mean the “noise” is bounded? To me, it seems the advantage of the proposed method come from being able to deal with outliers?}

\item \yao{-Why do we need superscript (ij) on T, R and t? Why don’t we use simpler notation?}

\item \yao{- The pairwise matching module operates on each object
pair in isolation.  — I do not understand this.}

\item \yao{one last comment for section 3 - we have already start to talk about weights $w_i$ in this section. However, the role of weights only become clear in section 4 (equation 1) so look at here it is really confusion.
}
\end{itemize}


\subsection{Variant I}

Given $T_{ij}^{\init}, w_{ij}^{\init}, (i,j)\in \set{E}$. Apply reweighted non-linear least squares for rotation and translation synchronizations. 

\begin{itemize}
\item Initialize $w_{ij,\textup{rot}}^{(0))}= w_{ij,\textup{trans}}^{(0)} = 1, (i,j)\in \set{E}$.
\item Perform rotation synchronization by taking $w_{ij, \textup{rot}}^{(k)}\cdot w_{ij}^{\init}, R_{ij}^{\init}, (i,j)\in \set{E}$ as input and outputs $R_i^{(k+1)}, 1\leq i \leq n$. This is done by applying formula (2) to formula (3) in Section 4.1. Perform translation synchronization by taking $w_{ij, \textup{trans}}^{(k)}\cdot w_{ij}^{\init}, R_{ij}^{\init}, \bs{t}_{ij}^{\init}, (i,j)\in \set{E}$ as input and outputs $\bs{t}_i^{(k+1)}, 1\leq i \leq n$. This is done by solving a linear system described in Equation (7).
\item Reweight $w_{ij,\textup{rot}}^{(k+1)}$ based on
$$
w_{ij,\textup{rot}}^{(k+1)} = \frac{\sigma_{rot}}{\sqrt{\sigma_{rot}^2 + \|R_{ij}^{\init}-R_j^{(k+1)}{R_i^{(k+1)}}^{T}\|_{\set{F}}^2}}.
$$
Reweight $w_{ij,\textup{trans}}^{(k+1)}$ based on
$$
w_{ij,\textup{trans}}^{(k+1)} = \frac{\sigma_{trans}}{\sqrt{\sigma_{trans}^2 + \|R_{ij}^{\init}\bs{t}_i^{(k+1)}+\bs{t}_{ij}^{\init}-\bs{t}_j^{(k+1)}\|^2}}.
$$
\end{itemize}
We set $\sigma_{rot} = 0.05$ and $\sigma_{trans} = 0.05$.

\subsection{Variant II}

Given $T_{ij}^{\init}, w_{ij}^{\init}, (i,j)\in \set{E}$. Apply reweighted non-linear least squares for rotation and translation synchronizations. 

\begin{itemize}
\item Initialize $w_{ij}^{(0))}=1, (i,j)\in \set{E}$.
\item Perform rotation synchronization by taking $w_{ij}^{(k)}\cdot w_{ij}^{\init}, R_{ij}^{\init}, (i,j)\in \set{E}$ as input and outputs $R_i^{(k+1)}, 1\leq i \leq n$. This is done by applying formula (2) to formula (3) in Section 4.1. Perform translation synchronization by taking $w_{ij}^{(k)}\cdot w_{ij}^{\init}, R_{ij}^{\init}, \bs{t}_{ij}^{\init}, (i,j)\in \set{E}$ as input and outputs $\bs{t}_i^{(k+1)}, 1\leq i \leq n$. This is done by solving a linear system described in Equation (7).
\item Reweight $w_{ij}^{(k+1)}$ based on
\begin{equation}
w_{ij}^{(k+1)} = \frac{\sigma}{\sqrt{\sigma^2 + r_{ij,\textup{rot}}^{(k+1)}+r_{ij,\textup{trans}}^{(k+1)}}}.
\label{Eq:2}
\end{equation}
where
$$
r_{ij,\textup{rot}}^{(k+1)} = \|R_{ij}^{\init}-R_j^{(k+1)}{R_i^{(k+1)}}^{T}\|^2_{\set{F}},
$$
and
$$
r_{ij,\textup{trans}}^{(k+1)} = \|R_{ij}^{\init}\bs{t}_i^{(k+1)}+\bs{t}_{ij}^{\init}-\bs{t}_j^{(k+1)}\|^2.
$$
\end{itemize}
We set $\sigma = 0.1$ and $\mu = 1$.

\subsection{Variant III}

Train a neural network that takes $\sqrt{r_{ij,rot}^{(k+1)}}$ and $\sqrt{r_{ij,trans}^{(k+1)}}$ as input and outputs $\frac{\sigma}{\sqrt{\sigma^2+r_{ij,rot}^{(k+1)}+r_{ij,trans}^{(k+1)}}}$
Replace the explicit weighting in (\ref{Eq:2}) by this neural network. 

\subsection{Variant IV}

Train the neural network to minimize
\begin{align}
\min\limits_{\theta}\sum\limits_{\set{S}\in \set{T}}
&\Big(\sum\limits_{1\leq i < j \leq |\set{S}|}\|R_j^{k_{\max}}{R_i^{k_{\max}}}^{T}-R_j^{\gt}{R_i^{\gt}}^{T}\|_{\set{F}}^2 \nonumber \\
& + \lambda \sum\limits_{i=1}^{|\set{S}|}\|\bs{t}_i^{k_{\max}}-\bs{t}_i^{\gt}\|^2\Big)
\end{align}

\subsection{Baseline V}

==> app_02_proof.bak.tex <==
\section{Proofs of Propositions}
\label{Section:Proofs:Propositions}

We organize this section as follows. In Section~\ref{Section:Connection:Laplacian:Stability}, we provide key lemmas regarding the eigen-decomposition of connection Laplacians, including stability of eigenvalues/eigenvectors and derivatives of eigenvectors with respect to elements of the connection Laplacian. In Section~\ref{Section:SO:Projection:Operator}, we provide key lemmas regarding the projection operator that maps the space of square matrices to the space of rotations.  Section~\ref{Section:Prop:4:1} to Section~\ref{Section:Prop:4:4} describe the proofs of all the propositions stated in the main paper. Finally, Section~\ref{Section:Proof:Lemma} provides proofs for new key lemmas introduced in this section.

\subsection{Eigen-Stability of Connection Laplacian}
\label{Section:Connection:Laplacian:Stability}

We begin with introducing the problem setting and notations in Section~\ref{Section:Key:Lemma:Notation}. We then present the key lemmas in Section~\ref{Section:Key:Lemmas}.

\subsubsection{Problem Setting and Notations}
\label{Section:Key:Lemma:Notation}

Consider we weighted graph $\set{G} = (\set{V}, \set{E})$ with $n$ vertices, i.e., $|\set{V}|=n$. We assume that $\set{G}$ is connected. With $w_{ij}>0$ we denote an edge weight associated with edge $(i,j)\in \set{E}$. Let $\overline{L}$ be the weighted adjacency matrix (Note that we drop $\bs{w}$ from the expression of $\overline{L}$ to make the notations uncluttered). It is clear that the leading eigenvector of $\overline{L}$ is $\frac{1}{\sqrt{n}}\bs{1}\in \R^n$, whose corresponding eigenvalue is zero. In the following, we shall denote the eigen-decomposition of $\overline{L}$ as
$$
\overline{L} = \overline{U}\overline{\Lambda}\overline{U}^{T},
$$
where
$$
\overline{U} = (\overline{\bs{u}}_2,\cdots, \overline{\bs{u}}_n) \ \textup{and} \ \overline{\Lambda} = \diag(\overline{\lambda}_2,\cdots, \overline{\lambda}_n)
$$
collect the remaining eigenvectors and their corresponding eigenvalues of $L(\bs{w})$, respectively. Our analysis will also use a notation that is closely related to the pseudo-inverse of $\overline{L}$:
\begin{equation}
\overline{L}_{t}^{+}:= \overline{U}(\overline{\Lambda} + t I_{n-1})^{-1} \overline{U}^{T}, \quad \forall |t| < \overline{\lambda}_2.
\end{equation}


Our goal is to understand the behavior of the leading eigenvectors of $\overline{L}\otimes I_k + E$\footnote{Note that when applying the stability results to the problem studied in this paper, we always use $k=3$. However, when assume a general $k$ when describing the stability results.} for a symmetric perturbation matrix $E\in \R^{nk\times nk}$, which is a $n\times n$ block matrix whose blocks are given by
$$
E_{ij} = \left\{
\begin{array}{cc}
0 & i = j \\
-w_{ij}N_{ij} & (i,j) \in \set{E}
\end{array}
\right.\
$$
where $N_{ij}$ is the perturbation imposed on $R_{ij}$. 


We are interested in $U\in \R^{nk\times k}$, which collects the leading $k$ eigenvectors of $\overline{L}\otimes I_k + E$ in its columns. With $\lambda_1\leq \lambda_2 \cdots \leq \lambda_k$, we denote the corresponding eigenvalues. Note that due to the property of connection Laplacian, $\lambda_i \geq 0,1\leq i \leq k$. Our goal is to 1) bound the eigenvalues $\lambda_i, 1\leq i \leq k$, and 2) to provide block-wise bounds between $U$ and $\frac{1}{\sqrt{n}}\bs{1}\otimes R$, for some rotation matrix $R\in SO(k)$. 

%To this end, we introduce a few notations. We shall first reformulate $N$ under the basis specified by $\frac{1}{\sqrt{n}}\bs{1}\otimes I_k$ and $\overline{U}\otimes I_k$:
%\begin{align*}
%E_{11} &:= \frac{1}{n}(\bs{1}\otimes I_k)^{T}N(\bs{1}\otimes I_k), \\
%E_{12} &:= \frac{1}{\sqrt{n}}(\bs{1}\otimes I_k)^{T}N(\overline{U}\otimes I_k),\\
%E_{21} &:= \frac{1}{\sqrt{n}}(\overline{U}\otimes I_k)^{T}N(\bs{1}\otimes I_k),\\
%E_{22} &:= (\overline{U}\otimes I_k)^{T}N(\overline{U}\otimes I_k).
%\end{align*}

Besides the notations introduced above that are related to Laplacian matrices, we shall also use a few matrix norms. With $\|\cdot\|$ and $\|\cdot\|_{\set{F}}$ we denote the spectral norm and Frobenius norm, respectively. Given a vector $\bs{v}\in \R^n$, we denote $\|\bs{v}\|_{\infty} = \max\limits_{1\leq i \leq n}|v_i|$ as the elementwise infinity norm.

\subsubsection{Key Lemmas}
\label{Section:Key:Lemmas}

This section presents a few key lemmas which will be used to establish main stability results regarding matrix eigenvectors and matrix eigenvalues. We begin with the classical result of the Weyl's inequality:
\begin{lem}
(\textbf{Eigenvalue stability}) For $1 \leq i \leq k$, we have
\begin{equation}
\lambda_i \leq \|E\|
\end{equation}
\label{Lemma:Eigenvalue:Stability}
\end{lem}
We proceed to describe tools for controlling the eigenvector stability. To this end, we shall rewrite $U$ as follows:
$$
U = \frac{1}{\sqrt{n}}\bs{1}\otimes X + Y.
$$
Our goal is to bound the deviation between $X$ and a rotation matrix and blocks of $Y$.

We begin with controlling $X$, which we again adopt a result described in \cite{DBLP:conf/icml/BajajGHHL18}:
\begin{lem}
(\textbf{Controlling $X$}\cite{DBLP:conf/icml/BajajGHHL18}) If
$$
\|E\|<\frac{\overline{\lambda}_2}{2},
$$
then there exists $Q \in SO(k)$\footnote{If not, we can always negate the last column of U.} such that
$$
\|X - Q\| \leq 1 - \sqrt{1 - \left(\frac{\|E\|}{\overline{\lambda}_2- \|E\|}\right)^2}.
$$
In particular,
$$
\|X - Q\| \leq \left(\frac{\|E\|}{\overline{\lambda} - \|E\|}\right)^2
$$
\label{Lemma:Eigenvector:L2:Stability}
\end{lem}

It remains to control the blocks of $Y$. We first state a formulation that expresses the column of $Y$ using a series:
\begin{lem}
Suppose $\|E\| < \frac{\overline{\lambda}_2}{2}$, then $\forall 1\leq j \leq k$,
\begin{equation}
Y \bs{e}_j^{(k)} = -\frac{1}{\sqrt{n}}\sum\limits_{l=1}^{\infty}\Big((\overline{L}_{-\lambda_j}^{+}\otimes I_k)E\Big)^l (\bs{1}\otimes X)\bs{e}_j^{(k)}.
\label{Y:expression}
\end{equation}
\label{Lemma:Y:Expression}
\end{lem}

The following lemma provides an explicit expression for computing the derivative of the leading eigenvectors of a connection Laplacian with its elements:
\begin{lem}
Let $L$ be an $N\times N$ non-negative definite matrix and its eigen-decomposition is
\begin{equation}
L=\sum_{i=1}^N \lambda_i \bs{u}_i\bs{u}_i^T
\label{eq:derivative:decomposition}
\end{equation}
where $0\leq \sigma_1\leq \sigma_2\leq \dots\sigma_N$.

Suppose $\sigma_{k}<\sigma_{k+1}$. Collect the eigenvectors corresponding to the smallest $k$ eigenvalues of $L$ as the columns of matrix $U_k$. Namely, $U_k=[\bs{u}_1,\dots,\bs{u}_k]$ where $\sigma_1,\dots,\sigma_k$ are the smallest $k$ eigenvelues of $L$.

Notice that $L$ can have different decompositions in (\ref{eq:derivative:decomposition}) when there are repetitive eigenvalues. But in our case that assumed $\sigma_k<\sigma_{k+1}$ we claim that $U_k U_k^T$ is unique under different possible decomposition of $L$ so that $\dd(U_kU_k^T)$ can be well defined and has an explicit expression
\begin{equation}
    \dd (U_kU_k^T)=\sum_{i=1}^k\sum_{j=k+1}^{N}\frac{\bs{u}_j^T\dd L\bs{u}_i}{\sigma_i-\sigma_j}(\bs{u}_i\bs{u}_j^T+\bs{u}_j\bs{u}_i^T)
\end{equation}
Moreover, the differentials of eigenvalues are
\begin{equation}
    \dd \sigma_i=\bs{u}_i^T\dd L\bs{u}_i.
    \label{eq:derivative:eigenvalue}
\end{equation}
\label{Lemma:Laplacian:Derivative}
\end{lem}

\subsection{Key Lemma Regarding the Projection Operator}
\label{Section:SO:Projection:Operator}

This section studies the projection operator which maps the space of square matrices to the space of rotation matrices. We begin with formally defining the projection operator as follows:

\begin{definition}
Suppose $det(M) > 0$. Let $M=\sum_{i=1}^n\sigma_i\bs{u}_i\bs{v}_i^T$ be the singular value decomposition of square matrix $M$ where $U=[\bs{u}_1,\dots,\bs{u}_1]$ and $V=[\bs{v}_1,\dots,\bs{v}_n]$ are both orthogonal matrices, and all coefficients $\sigma_i$ are non-negative. Then we define the rotation approximation of $M$ as
$$
R(M):=\sum_{i=1}^n\bs{u}_i\bs{v}_i^T=UV^T.
$$
It is clear $R(M)$ is a rotation since 1) both $U$ and $V^T$ are rotations, and 2) $\det(UV^{T}) > 0$.
\label{def:rotation}
\end{definition}

\begin{lem}
Let $A\in\mathbb{R}^{nk\times k}$ be a block matrix of form
$$
A=\begin{bmatrix}
A_1\\
\vdots\\
A_n
\end{bmatrix}
$$
where $A_i\in\mathbb{R}^{k\times k}$. Use $a_{ij}$ to denote the element on position $i,j$ in $A$. Then we have
$$
\sum_{i=1}^n\|A_i\|^2\leq k\|A\|^2
$$
\label{Lemma:Block:Norm}
\end{lem}
\noindent\textsl{Proof:} See Section~\ref{Section:Proof:Lemma}. \qed

We then present the following key lemma regarding the stability of the projection operator:
\begin{lem}
Let $M$ be a square matrix and $\epsilon=\|M-I\|$. Suppose $\epsilon< \frac{1}{3}$, then
$$
\|R(M)-I\|\leq \epsilon+\epsilon^2.
$$
\label{Lemma:Projection:Stability}
\end{lem}
\noindent\textsl{Proof:} See Section~\ref{Section:Proof:Lemma}. \qed


\begin{lem}
Regarding $R(M)$ as a function about $M$, then the differential of $R(M)$ would be
$$
\dd R(M)=\sum_{i\neq j}\frac{\bs{u}_i^T\dd M\bs{v}_j-\bs{u}_j^T\dd M\bs{v}_i}{\sigma_i+\sigma_j}\bs{u}_i\bs{v}_j^T
$$
where all notations follow Defintion (\ref{def:rotation}).
\label{prop:derivative:single_rotation}
\end{lem}


\subsection{Proof of Prop. 4.1}
\label{Section:Prop:4:1}

We first present a general lemma regarding the stability of the connection Laplacian $L\in \R^{kn\times kn}$, which is an $n\times n$ block matrix. Suppose each observation is given by
$$
R_{ij} = R_j^{\star}{R_i^{\star}}^T + E_{ij}, \quad 1\leq i < j \leq n.
$$
We decompose the connection Laplacian as the sum of two components:
$$
L = L^{\star} + N,
$$
where
$$
L^{\star}_{ji} = \left\{
\begin{array}{cc}
\sum_{l\neq i}w_{il} & i = j \\
-w_{ij}R_j^{\star}{R_i^{\star}}^T & j > i
\end{array}
\right.\,\ N_{ji} = \left\{
\begin{array}{cc}
0 & i = j \\
-w_{ij}E_{ij} & j > i
\end{array}
\right.\ .
$$


\noindent\textbf{Completion of the proof of Prop. 4.1:}

\qed

\subsection{Proof of Prop. 4.2}
\label{Section:Prop:4:2}

\subsection{Proof of Prop. 4.3}
\label{Section:Prop:4:3}

Applying Lemma~\ref{prop:derivative:single_rotation} we have
\begin{align}
\dd R_i=\sum_{1\leq s,t\leq k}\frac{{\bs{v}^{(i)}_s}^T\dd U_i\bs{w}_t^{(i)}-{\bs{v}_t^{(i)}}^T\dd U_i\bs{w}_s^{(i)}}{\sigma_s^{(i)}+\sigma_t^{(i)}}\bs{v}_s^{(i)}{\bs{w}_t^{(i)}}^T.
\end{align}

We further divide the computation of $\dd U_i$ into two parts. Consider the $j$-th column of $\dd U_i$:
\begin{align}
    \dd U_i\bs{e}_j^{(k)}&=({\bs{e}_i^{(n)}}^T\otimes I_k)\dd U\bs{e}_j^{(k)}\nonumber\\
    &=({\bs{e}_i^{(n)}}^T\otimes I_k)\dd \bs{u}_j\nonumber\\
    &=({\bs{e}_i^{(n)}}^T\otimes I_k)\sum_{l\neq j}\bs{u}_l\frac{\bs{u}_j^T\dd L\bs{u}_l}{\lambda_j-\lambda_l}\nonumber\\
    &=({\bs{e}_i^{(n)}}^T\otimes I_k)\Big(\sum_{\substack{l=1\\l\neq j}}^k\frac{\bs{u}_j^T\dd L\bs{u}_l}{\lambda_j-\lambda_l}\bs{u}_l+\nonumber\\
    &\qquad\sum_{l=k+1}^{kn}\frac{\bs{u}_j^T\dd L\bs{u}_l}{\lambda_j-\lambda_l}\bs{u}_l\Big)\nonumber\\
    &=\dd U_i^{(inner)}\bs{e}_j^{(k)}+\dd U_i^{(outer)}\bs{e}_j^{(k)}
\end{align}
where
\begin{align}
\dd U_i^{(inner)}\bs{e}_j^{(k)}&=({\bs{e}_i^{(n)}}^T\otimes I_k)\sum_{\substack{l=1\\l\neq j}}^k\frac{\bs{u}_l\bs{u}_l^{T}}{\lambda_j-\lambda_l}\dd L\bs{u}_j
\label{eq:derivative:20}
\\
&=\sum_{\substack{l=1\\l\neq j}}^k (U_i\bs{e}_l^{(k)})\frac{\bs{u}_l\bs{u}_l^T}{\lambda_j-\lambda_l}\dd L\bs{u}_j\\
\dd U_i^{(outer)}\bs{e}_j^{(k)} &= ({\bs{e}_i^{(n)}}^T\otimes I_k)\sum_{l=k+1}^{kn}\frac{\bs{u}_l\bs{u}_l^T}{\lambda_j-\lambda_l}\dd L\bs{u}_j
\label{eq:derivative:17}
\end{align}
In (\ref{eq:derivative:20}) we use the fact that $({\bs{e}_i^{(n)}}^T\otimes I_k)\bs{u}_l$ is just $U_i\bs{e}_l^{(k)}$ by definition of $U_i$.

Since $\dd R_i$ is linear about $\dd U_i$, we can divide $\dd R_i$ similarly:
\begin{align}
&\dd R_i = \dd R_{i}^{(inner)}+\dd R_{i}^{(outer)}\nonumber\\
&\dd R_i^{(inner)}:=\nonumber\\
&\sum_{1\leq s,t\leq k}\frac{{\bs{v}^{(i)}_s}^T\dd U_i^{(inner)}\bs{w}_t^{(i)}-{\bs{v}_t^{(i)}}^T\dd U_i^{(inner)}\bs{w}_s^{(i)}}{\sigma_s^{(i)}+\sigma_t^{(i)}}\bs{v}_s^{(i)}{\bs{w}_t^{(i)}}^T
\label{eq:derivative:15}
\\
&\dd R_i^{(outer)}:=\nonumber\\
&\sum_{1\leq s,t\leq k}\frac{{\bs{v}^{(i)}_s}^T\dd U_i^{(outer)}\bs{w}_t^{(i)}-{\bs{v}_t^{(i)}}^T\dd U_i^{(outer)}\bs{w}_s^{(i)}}{\sigma_s^{(i)}+\sigma_t^{(i)}}\bs{v}_s^{(i)}{\bs{w}_t^{(i)}}^T
\label{eq:derivative:16}
\end{align}

Then the object derivative can be written as
\begin{align}
\dd (R_i R_j^T)&=\dd R_iR_j^T+R_i{\dd R_j}^T\nonumber\\
&=\dd R_i^{(inner)} R_j^T+R_i{\dd R_j^{(inner)}}^T\nonumber\\
&\quad +\dd R_i^{(outer)}R_j^T+R_i\dd {R_j^{(outer)}}^T.
\label{eq:derivative:18}
\end{align}
From (\ref{eq:derivative:16}) and (\ref{eq:derivative:17}) it can be easily checked that the formula (\ref{eq:derivative:14}) that we want to prove is just (\ref{eq:derivative:18}) except the extra terms $\dd R_i^{(inner)}R_j^T+R_i\dd {R_j^{(inner)}}^T$. Hence in the remaining proof it suffices to show that
$$
\dd R_i^{(inner)}R_j^T+R_i\dd {R_j^{(inner)}}^T=0.
$$

To this end, we define a $k$-by-$k$ auxiliary matrix $C$ as
$$
C_{lj}=\frac{\bs{u}_j^T\dd L\bs{u}_l}{\lambda_j-\lambda_l}
$$
for all $l\neq j$ and $C_{jj}=0$. Since $L$ is symmetric, $C$ would be skew-symmetric that means $C+C^T=0$. Fist of all notice that
$$
\dd U_i^{(inner)}=\sum_{\substack{l=1\\l\neq k}}^k (U_i\bs{e}_l^{(k)})\frac{\bs{u}_j^T\dd L\bs{u}_l}{\lambda_j-\lambda_l}=U_i C.
$$
Also it is clear that
$$
{\bs{v}_s^{(i)}}^T U_i=\sigma_s\bs{w}_s^T
$$
by using simple properties of SVD. In this way from (\ref{eq:derivative:15}) we have
\begin{align}
\dd R_i^{(inner)}&=\sum_{1\leq s,t\leq k}\frac{\sigma_s{\bs{w}_s^{(i)}}^TC\bs{w}_t^{(i)}-\sigma_t{\bs{w}_t^{(i)}}^TC\bs{w}_s^{(i)}}{\sigma_s^{(i)}+\sigma_t^{(i)}}\bs{v}_s^{(i)}{\bs{w}_t^{(i)}}^T\label{eq:19:1}\\
&=\sum_{1\leq s,t\leq k}{\bs{w}_s^{(i)}}^TC\bs{w}_t^{(i)}\bs{v}_s^{(i)}{\bs{w}_t^{(i)}}^T\label{eq:19:2}\\
&=\sum_{1\leq s,t\leq k}{\bs{v}_s^{(i)}}{\bs{w}_s^{(i)}}^TC\bs{w}_t^{(i)}{\bs{w}_t^{(i)}}^T\label{eq:19:3}\\
&={V^{(i)}}{W^{(i)}}^TC\label{eq:19:4}\\
&=R_iC.
\label{eq:derivative:19}
\end{align}
In the derivations above, we used the fact that $C$ is a skew-symmetric matrix for deriving the first equality (\ref{eq:19:1}). In addition, we used the fact that ${\bs{v}_s^{(i)}}^TC\bs{v}_t^{(i)}$ is a scalar for deriving the second equality (\ref{eq:19:2}). When deriving (\ref{eq:19:3}), we used the expansion of $U^{(i)}{V^{(i)}}^T$ and the fact that $\{\bs{v}_1^{(i)},\dots,\bs{v}_k^{(i)}\}$ form orthonormal basis:
$$
U^{(i)}{V^{(i)}}^T=\sum_{s=1}^k\bs{u}_s^{(i)}{\bs{v}_s^{(i)}}^T,\ I=\sum_{t=1}^k \bs{v}_s^{(i)}{\bs{v}_s^{(i)}}^T.
$$
(\ref{eq:19:4}) uses the definition of $R_i$. Finally, plugging (\ref{eq:derivative:19}) into (\ref{eq:derivative:18}) gives
$$
\dd R_i^{(inner)} R_j^T+R_i{\dd R_j^{(inner)}}^T=R_iC R_j^T+R_iC^TR_j^T=0,
$$
which completes our proof.
\qed

\subsection{Proof of Prop. 4.4}
\label{Section:Prop:4:4}

\subsection{Proofs of Key Lemmas}
\label{Section:Proof:Lemma}

\subsubsection{Proof of Lemma~\ref{Lemma:Y:Expression}}

We first introduce the following notations, which essentially express $E$ in the coordinate system spanned by $\frac{1}{\sqrt{n}}(\bs{1}\otimes I_k)$ and $\overline{U}\otimes I_k$:
\begin{align*}
E_{11}: & = \frac{1}{n}(\bs{1}\otimes I_k)^{T}E(\bs{1}\otimes I_k), \\
E_{12}: & = \frac{1}{\sqrt{n}}(\bs{1}\otimes I_k)^{T}E(\overline{U}\otimes I_k),\\
E_{21}: & = \frac{1}{\sqrt{n}}(\overline{U}\otimes I_k)^{T}E(\bs{1}\otimes I_k),
E_{22}: & = (\overline{U}\otimes I_k)^{T}E(\overline{U}\otimes I_k).
\end{align*}

Let $Y: = (U\otimes I_k)\overline{Y}$. Substituting $U = \frac{1}{\sqrt{n}}(\bs{1}\otimes I_k) + (\overline{U}\otimes I_k)\overline{Y}$ into 
$$
(\overline{L}\otimes I_k+E)U = U\Lambda,
$$
we obtain
$$
(\overline{L}\otimes I_k+E)(\frac{1}{\sqrt{n}}(\bs{1}\otimes I_k) + (\overline{U}\otimes I_k)\overline{Y})=(\frac{1}{\sqrt{n}}(\bs{1}\otimes I_k) + (\overline{U}\otimes I_k)\overline{Y})\Lambda.
$$
Multiply both sides by $(U\otimes I_k)^{T}$, it follows that
$$
E_{21}X + \overline{\Lambda}\overline{Y} + E_{22}\overline{Y} = \overline{Y}\Lambda.
$$
Since $\|E\| < \frac{\overline{\lambda}_2}{2}$, we have
\begin{align*}
Y\bs{e}_{j}^{(k)} &:= (\overline{U}\otimes I_k)\overline{Y}\bs{e}_j^{(k)} \\
& = -(\overline{U}\otimes I_k)(\overline{\Lambda}-\lambda_j-E_{22})^{-1}E_{21}X\bs{e}_j^{(k)} \\
& = -\sum\limits_{l=0}^{\infty}(\overline{U}\otimes I_k)\big((\overline{\Lambda}-\lambda_j)^{-1}E_{22}\big)^l(\overline{\Lambda}-\lambda_j)^{-1}E_{21}X\bs{e}_j^{(k)} \\
& = -\sum\limits_{l=1}^{\infty}(\overline{U}\otimes I_k)(\overline{\Lambda}-\lambda_j)^{-1}E (\overline{U}\otimes I_k)(\overline{\Lambda}-\lambda_j)^{-1}E_{21}X\bs{e}_j^{(k)}
\end{align*}
\qed
\subsubsection{Proof of Lemma~\ref{Lemma:Laplacian:Derivative}} 
Let
\begin{align*}
    L=\sum_{i=1}^N\sigma_i\bs{u}_i\bs{u}_i^T=\sum_{i=1}^N\sigma_i\bs{u}'_i\bs{u}'^{T}_i
\end{align*}
be two different decompositions of $L$. It can be written in matrix form
$$
L=U\Lambda U^T=U'\Lambda U'^T
$$
where $U=[\bs{u}_1,\dots,\bs{u}_N]$, $\Lambda=\diag(\sigma_1,\dots,\sigma_N)$, $U'=[\bs{u}'_1,\dots,\bs{u}_N]$. Then we have
$$
(U'^TU)\Lambda=\Lambda (U'^TU)
$$

Let $A=U'^TU$ and the element of position $(i,j)$ on $A$ be $a_{ij}$, then we have
$$
a_{ij}\sigma_j=\sigma_ia_{ij},
$$
which means $a_{ij}=0$ for all $\sigma_i\neq \sigma_j$.

Since we have assumed $\sigma_1\leq \dots\leq \sigma_k<\sigma_{k+1}\leq\dots\leq \sigma_N$, the matrix $A$ would have form
$$
\begin{bmatrix}
A_{k,k} & O_{k,N-k}\\
O_{N-k,k} & A_{N-k,N-k}
\end{bmatrix}.
$$

But we have known that $A$ is an orthogonal matrix, thus $A_{k,k}$ is also an orthogonal matrix. In this way $A_{k,k}=U'^T_kU_k$ can be rewritten as
$$
U_k=U'_kA_{k,k}
$$
and furthermore we have
$$
U_kU_k^T=U_k'(A_{k,k}A_{k,k}^T)U'^T_k=U_k'U'^T_k.
$$

Since eigen-decomposition is a special case of SVD when dealing with symmetric matrix, (\ref{eq:derivative:9}) gives
\begin{align*}
\dd \bs{u}_i&=\sum_{j\neq i}\frac{\sigma_i \bs{u}_j^T\dd L\bs{u}_i+\sigma_j\bs{u}_i^T\dd L\bs{u}_j}{\sigma_i^2-\sigma_j^2}\bs{u}_j\\
&=\sum_{j\neq i}\frac{\bs{u}_i^T\dd M\bs{u}_j}{\sigma_i-\sigma_j}\bs{u}_j
\end{align*}
in which we used the fact that $\dd L$ is also symmetric in the last step.

Finally the differential of $U_kU_k^T$ can be written as
\begin{align*}
    &\dd(U_k U_k^T)\\
    =&\dd\left(\sum_{i=1}^k\bs{u}_i\bs{u}_i^T\right)\\
    =&\sum_{i=1}^k(\dd \bs{u}_i\bs{u}_i^T+\bs{u}_i\dd\bs{u}_i^T)\\
    =&\sum_{i=1}^k\sum_{\substack{j=1\\j\neq i}}^N\frac{\bs{u}_i^T\dd M\bs{u}_j}{\sigma_i-\sigma_j}(\bs{u}_j\bs{u}_i^T+\bs{u}_i \bs{u}_j^T)\\
    =&\sum_{i=1}^k\sum_{j=k+1}^N\frac{\bs{u}_i^T\dd M\bs{u}_j}{\sigma_i-\sigma_j}(\bs{u}_j\bs{u}_i^T+\bs{u}_i \bs{u}_j^T)+\\
    &\sum_{i=1}^k\sum_{j=i+1}^k\left(\frac{\bs{u}_i^T\dd M\bs{u}_j}{\sigma_i-\sigma_j}+\frac{\bs{u}_i^T\dd M\bs{u}_j}{\sigma_j-\sigma_i}\right)(\bs{u}_j\bs{u}_i^T+\bs{u}_i \bs{u}_j^T)\\
    =&\sum_{i=1}^k\sum_{j=k+1}^N\frac{\bs{u}_i^T\dd M\bs{u}_j}{\sigma_i-\sigma_j}(\bs{u}_j\bs{u}_i^T+\bs{u}_i \bs{u}_j^T)
\end{align*}

As for formula (\ref{eq:derivative:eigenvalue}), taking differential of equation $L\bs{u}_i=\sigma_i\bs{u}_i$ we obtain
$$
\dd L\bs{u}_i+L\dd\bs{u}_i=\dd\sigma_i\bs{u}_i+\sigma_i\dd\bs{u}_i
$$

Left multiply both sides by $\bs{u}_i^T$ and notice $\bs{u}_i^T\bs{u}_i=1$, $L\bs{u}_i=\sigma_i\bs{u}_i$ and $\bs{u}_i^T\dd\bs{u}_i=0$, the equation above can be simplified to
$$
\dd\sigma_i=\bs{u}_i^T\dd L\bs{u}_i.
$$
\qed

\subsubsection{Proof of Lemma~\ref{Lemma:Block:Norm}} 

It is well-known that $\|X\|\leq \|X\|_F$ for any matrix $X$ where $\|\cdot\|_F$ represents the Frobenius norm. Thus
\begin{align*}
k\|A\|^2&= \sum_{j=1}^k\|A\|^2\geq\sum_{j=1}^k\sum_{i=1}^{kn}a_{ij}^2\\
    &=\sum_{i=1}^{kn}\sum_{j=1}^ka_{ij}^2=\sum_{i=1}^n \|A_{i}\|_F^2\\
    &\geq \sum_{i=1}^n \|A_i\|
\end{align*}
completes our proof.
\qed

\subsubsection{Proof of Lemma~\ref{Lemma:Projection:Stability}} 

Suppose $M=\sum_{i=1}^n\sigma_i\bs{u}_i\bs{v}_i^T$ is the SVD decomposition of $M$.  By definition of $R(\cdot)$,
$$R(M)=\sum_{i=1}^n\bs{u}_i\bs{v}_i^T.$$
First we have an simple lower bound on $\epsilon$:
\begin{equation}
\epsilon=\|M-I\|\geq |(M-I)\bs{v_i}|=|\sigma_i-1|.
\label{eq:derivative:12}
\end{equation}
It is enough to show that for any unit vector $\bs{p}\in\mathbb{R}^{n}$ we have
\begin{equation}
\|R(M)\bs{p}-\bs{p}\|\leq (1+\epsilon)\|M\bs{p}-\bs{p}\|.
\label{eq:derivative:11}
\end{equation}
In fact, if (\ref{eq:derivative:11}) is true, then
\begin{align*}
\|R(M)-I\|&=\max_{|\bs{p}|=1}\|R(M)\bs{p}-\bs{p}\|\\
&\leq \max_{|\bs{p}=1}(1+\epsilon)\|M\bs{p}-\bs{p}\|\\
&\leq (1+\epsilon)\epsilon\textup{\quad (by definition of $\epsilon$)}.
\end{align*}

By noting $\{\bs{v}_1,\dots,\bs{v}_n\}$ are a set of basis on $\mathbb{R}^n$, we can decompose $R(M)$ and $M$ into
\begin{align*}
R(M)\bs{p}-\bs{p}&=\sum_{i=1}^n\bs{u}_i\bs{v}_i^T\bs{p}-\sum_{i=1}^n\bs{v}_i(\bs{v}_i^T\bs{p})\\
&=\sum_{i=1}^n(\bs{u}_i-\bs{v}_i)(\bs{v}_i^T\bs{p})\\
M\bs{p}-\bs{p}&=\sum_{i=1}^n\sigma_i\bs{u}_i\bs{v}_i\bs{p}-\sum_{i=1}^n\bs{v}_i(\bs{v}_i^T\bs{p})\\
&=\sum_{i=1}^n(\sigma_i\bs{u}_i-\bs{v}_i)(\bs{v}_i^T\bs{p})
\end{align*}
To prove (\ref{eq:derivative:11}), it suffices to show that
$$
|\bs{u}_i-\bs{v}_i|\leq (1+\epsilon)|\sigma_i\bs{u}_i-\bs{v}_i|.
$$
Let $\delta=\bs{u}_i^T\bs{v}_i$. The case that $\bs{u}_i=\bs{v}_i$ is trivial. Also, if $\sigma_i=0$, then $\epsilon\geq 1$ and the resulting inequality
$$
|\bs{u}_i-\bs{v}_i|\leq 2|\bs{v}_i|
$$
is trivial. Thus we can always assume $|\sigma \bs{u}_i-\bs{v}_i|\neq 0$ and $\sigma_i>0$. Then
by the laws of cosines we have
\begin{align}
\frac{|\bs{u}_i-\bs{v}_i|}{|\sigma_i\bs{u}_i-\bs{v}_i|}&=\sqrt{\frac{2-2\delta}{1+\sigma_i^2-2\sigma_i\delta}}\nonumber\\
&=\sqrt{\sigma_i^{-1}+\frac{2-(\sigma_i^{-1}+\sigma_i)}{1+\sigma_i^2-2\sigma_i\delta}}
\label{eq:derivative:13}
\end{align}
In (\ref{eq:derivative:13}) it is clear that $2-(\sigma_i^{-1}+\sigma_i)\leq 0$ and $1+\sigma_i^2\geq 2\sigma_i\delta$. Hence by monotonicity (\ref{eq:derivative:13}) reaches its maximum when $\delta=-1$ and then
$$
\frac{|\bs{u}_i-\bs{v}_i|}{|\sigma_i\bs{u}_i-\bs{v}_i|}\leq \frac{2}{1+\sigma_i}=1+\frac{1-\sigma_i}{1+\sigma_i}\leq 1+|\sigma_i-1|\leq 1+\epsilon
$$


\subsubsection{Proof of Lemma~\ref{prop:derivative:single_rotation}} 

For the sake of brevity we simply write $R$ instead of $R(M)$ in the following proof. It is easy to see that
$$
M\bs{v}_i=\sigma_i\bs{u}_i\quad \bs{u}_i^TM=\sigma_i\bs{v}_i^T
$$
for $i=1,\dots,n$. Taking the differential on both sides we obtain
\begin{equation}
\dd M\bs{v}_i+M\dd\bs{v}_i=\dd\sigma_i\bs{u}_i+\sigma_i\dd\bs{u}_i
\label{eq:derivative:1}
\end{equation}
\begin{equation}
\dd\bs{u}_i^TM+\bs{u}_i^T\dd M=\dd\sigma_i\bs{v}_i^T+\sigma_i\dd\bs{v}_i^T
\label{eq:derivative:2}
\end{equation}

Left multiplying both sides of (\ref{eq:derivative:1}) by $\bs{u}_j$ with $j\neq i$ and observing that $\bs{u}_j^T\bs{u}_i=0$ we obtain

\begin{equation}
\bs{u}_j^T\dd M\bs{v}_i+\bs{u}_j^TM\dd\bs{v}_i=\sigma_i\bs{u}_j^T\dd \bs{u}_i
\label{eq:derivative:3}
\end{equation}
Similarly right multiplying both sides of (\ref{eq:derivative:2}) by $\bs{v}_j^T$ with $j\neq i$ gives

\begin{equation}
\dd\bs{u}_i^TM\bs{v}_j+\bs{u}_i^T\dd M\bs{v}_j=\sigma_i\dd \bs{v}_{i}^T \bs{v}_j
\label{eq:derivative:4}
\end{equation}

Since $\bs{u}_j^TM=\sigma_j v_j^T,\ Mv_j=\sigma_j\bs{u}_j^T$, we have
\begin{equation}
\bs{u}_j^T\dd M\bs{v}_i+\sigma_j \bs{v}_j^T\dd\bs{v}_i=\sigma_i\bs{u}_j^T\dd \bs{u}_i
\label{eq:derivative:5}
\end{equation}
\begin{equation}
\dd\bs{u}_i^T\sigma_j\bs{u}_j+\bs{u}_i^T\dd M\bs{v}_j=\sigma_i\dd \bs{v}_{i}^T \bs{v}_j
\label{eq:derivative:6}
\end{equation}
for all $i\neq j$.

Observe that $\bs{u}_j^T\dd \bs{u}_i=\dd\bs{u}_i^T\bs{u}_j,\ \bs{v}_j^T\dd \bs{v}_i=\dd \bs{v}_i^T\bs{v}_j$. Combining (\ref{eq:derivative:5}) and (\ref{eq:derivative:6}) and regarding them as a linear equation group about $\bs{u}_j^T\dd\bs{u}_i$ and $\bs{v}_j^T\dd\bs{v}_i$ they can be solved out as

\begin{equation}
\bs{u}_j^T\dd\bs{u}_i=\frac{\sigma_i\bs{u}_j^T\dd M\bs{v}_i+\sigma_j\bs{u}_i^T\dd M\bs{v}_j}{\sigma_i^2-\sigma_j^2}
\label{eq:derivative:7}
\end{equation}
\begin{equation}
\bs{v}_j^T\dd \bs{v}_i=\frac{\sigma_i\bs{u}_i^T\dd M\bs{v}_j+\sigma_j\bs{u}_j^T\dd M\bs{v}_i}{\sigma_i^2-\sigma_j^2}
\label{eq:derivative:8}
\end{equation}

Since $\bs{u}_i^T\bs{u}_i=\|\bs{u}_i\|=1$, we have $\bs{u}_i^T\dd \bs{u}_i=0$. As $\{\bs{u}_1,\dots,\bs{u}_n\}$ form a set of orthogonal basis of $\mathbb{R}^n$, we can write $\bs{u}_i$ as
\begin{equation}
\dd\bs{u}_i=\sum_{j\neq i}\frac{\sigma_i\bs{u}_j^T\dd M\bs{v}_i+\sigma_j\bs{u}_i^T\dd M\bs{v}_j}{\sigma_i^2-\sigma_j^2}\bs{u}_j
\label{eq:derivative:9}
\end{equation}
Similarly for $\dd \bs{v}_i$ we have
\begin{equation}
\dd\bs{v}_i=\sum_{j\neq i}\frac{\sigma_i\bs{u}_i^T\dd M\bs{v}_j+\sigma_j\bs{u}_j^T\dd M\bs{v}_i}{\sigma_i^2-\sigma_j^2}\bs{v}_j
\label{eq:derivative:10}
\end{equation}

Finally we can write $\dd R$ as
\begin{align*}
\dd R&=\sum \bs{u}_i\dd \bs{v}_i^T+\sum \dd\bs{u}_i\bs{v}_i^T\\
&=\sum_{i\neq j}\frac{\sigma_i\bs{u}_i^T\dd M\bs{v}_j+\sigma_j\bs{u}_j^T\dd M\bs{v}_i}{\sigma_i^2-\sigma_j^2}\bs{u}_i\bs{v}_j^T\\
&\quad+\sum_{i\neq j}\frac{\sigma_i\bs{u}_j^T\dd M\bs{v}_i+\sigma_j\bs{u}_i^T\dd M\bs{v}_j}{\sigma_i^2-\sigma_j^2}\bs{u}_j\bs{v}_i^T\\
&=\sum_{i\neq j}\frac{(\sigma_i-\sigma_j)\bs{u}_i^T\dd M\bs{v}_j-(\sigma_i-\sigma_j)\bs{u}_j^T\dd M\bs{v}_i}{\sigma_i^2-\sigma_j^2}\bs{u}_i\bs{v}_j^T\\
&=\sum_{i\neq j}\frac{\bs{u}_i^T\dd M\bs{v}_j-\bs{u}_j^T\dd M\bs{v}_i}{\sigma_i+\sigma_j}\bs{u}_i\bs{v}_j^T
\end{align*}
\qed 

==> app_03_more_experiments.bak.tex <==
\section{Additional Experiments}
\label{Section:Additional:Experiments}

\begin{figure*}
\setlength\tabcolsep{1.75pt}
\begin{tabular}{cccc}
Ground Truth & RotAvg & Geometric Registration & Our Approach \\
\includegraphics[width=0.24\textwidth]{Figures/Appendix/gt_05989.png}
&
\includegraphics[width=0.24\textwidth]{Figures/Appendix/SO3_05989.png}
&
\includegraphics[width=0.24\textwidth]{Figures/Appendix/multiway_05989.png}
&
\includegraphics[width=0.24\textwidth]{Figures/Appendix/network_05989.png}
\\
\includegraphics[width=0.24\textwidth]{Figures/Appendix/gt_06031.png}
&
\includegraphics[width=0.24\textwidth]{Figures/Appendix/SO3_06031.png}
&
\includegraphics[width=0.24\textwidth]{Figures/Appendix/multiway_06031.png}
&
\includegraphics[width=0.24\textwidth]{Figures/Appendix/network_06031.png}
\\
\includegraphics[width=0.24\textwidth]{Figures/Appendix/gt_06283.png}
&
\includegraphics[width=0.24\textwidth]{Figures/Appendix/SO3_06283.png}
&
\includegraphics[width=0.24\textwidth]{Figures/Appendix/multiway_06283.png}
&
\includegraphics[width=0.24\textwidth]{Figures/Appendix/network_06283.png}
\\
\includegraphics[width=0.24\textwidth]{Figures/Appendix/gt_06198.png}
&
\includegraphics[width=0.24\textwidth]{Figures/Appendix/SO3_06198.png}
&
\includegraphics[width=0.24\textwidth]{Figures/Appendix/multiway_06198.png}
&
\includegraphics[width=0.24\textwidth]{Figures/Appendix/network_06198.png}
\\
\includegraphics[width=0.24\textwidth]{Figures/Appendix/gt_00286.png}
&
\includegraphics[width=0.24\textwidth]{Figures/Appendix/SO_00286.png}
&
\includegraphics[width=0.24\textwidth]{Figures/Appendix/multiway_00286.png}
&
\includegraphics[width=0.24\textwidth]{Figures/Appendix/network_00286.png}
\\
\includegraphics[width=0.24\textwidth]{Figures/Appendix/gt_05333.png}
&
\includegraphics[width=0.24\textwidth]{Figures/Appendix/SO3_05333.png}
&
\includegraphics[width=0.24\textwidth]{Figures/Appendix/multiway_05333.png}
&
\includegraphics[width=0.24\textwidth]{Figures/Appendix/network_05333.png}
\\
\includegraphics[width=0.24\textwidth]{Figures/Appendix/gt_01682.png}
&
\includegraphics[width=0.24\textwidth]{Figures/Appendix/SO3_01682.png}
&
\includegraphics[width=0.24\textwidth]{Figures/Appendix/multiway_01682.png}
&
\includegraphics[width=0.24\textwidth]{Figures/Appendix/network_01682.png}
\\
\hline 
\end{tabular}
\caption{\small{For each block, we show the results of our approach (row I), Rotation Averaging~\protect\cite{chatterjee2018robust}+Translation Sync.~\protect\cite{DBLP:conf/nips/HuangLBH17}~ (row II), Geometric  Registration~\protect\cite{conf/cvpr/ChoiZK15} (row III), and Ground Truth (row IV). The left four scenes are from Redwood and the right two scenes are from Scannet.}}
\label{Figure:More:Results}
\vspace{-0.15in}
\end{figure*}
